Purely viscous acoustic propulsion of bimetallic rods

Synthetic microswimmers offer models for cell motility and their tunability makes them promising candidates for biomedical applications. Here we measure the acoustic propulsion of bimetallic micro-rods that, when trapped at the nodal plane of a MHz acoustic resonator, swim with speeds of up to 300 microns per second. While past acoustic streaming models predict speeds that are more than one order of magnitude smaller than our measurements, we demonstrate that the acoustic locomotion of the rods is driven by a viscous, non-reciprocal mechanism relying on shape anisotropy akin to that used by swimming cells and that reproduces our data with no adjustable parameters.

==> bib_rods.tex <==
@article{Ahmed2015,
	author = {D. Ahmed and M. Lu and A. Nourhani and P.E. Lammert and Z. Stratton and H.S. Muddana and V.H. Crespi and T.J. Huang},
	title = {Selectively manipulable acoustic-powered microswimmers},
	journal = {Scientific Reports},
	title = {2015},
	volume = {5},
	pages = {9744}
	}

@article{Ahmed2014,
	author = {S. Ahmed and D.T. Gentekos and C.A. Fink and T.E. Mallouk},
	title = {Self-Assembly of Nanorod Motors into Geometrically Regular Multimers and Their Propulsion by 					Ultrasound},
	journal = {ACS Nano},
	volume = {8},
	number = {11},
	pages = {11053-11060},
	year = {2014}
	}

@article{Ahmed2016,
	author = {S. Ahmed and W. Wang and L. Bai and D.T. Gentekos and M. Hoyos and T.E. Mallouk},
	title = {Density and Shape Effects in the Acoustic Propulsion of Bimetallic Nanorod Motors},
	journal = {ACS Nano},
	volume = {10},
	number = {4},
	pages = {4763-4769},
	year = {2016}
	}

@article{Bruus2012,
	title = {Acoustofluidics 2: Perturbation theory and ultrasound resonance modes}, 
	author = {H. Bruss},
	journal = {Lab Chip},
	volume = {12},
	pages = {20--28},
	year = {2012}
	}
	
@article{Collis2017, 
	title={Autonomous propulsion of nanorods trapped in an acoustic field}, 
	volume={825},
	journal={Journal of Fluid Mechanics}, 
	publisher={Cambridge University Press}, 
	author={J. Collis and  F. Jesse and D. Chakraborty and J.E. Sader},
	year={2017}, 
	pages={29--48}
	}

@article{Esteban2016,
	author = {B. Esteban-Fern\'andez$\;$de$\;$\'Avila and C. Angell and F. Soto and M.A. Lopez-Ramirez,
	and D.F. B\'aez and S. Xie and J. Wang and Y. Chen},
	title = {Acoustically {P}ropelled {N}anomotors for {I}ntracellular si{RNA} {D}elivery},
	journal = {ACS Nano},
	volume = {10},
	number = {5},
	pages = {4997-5005},
	year = {2016}
	}
	
@article{Kaynak2017, 
	author = {M. Kaynak and A. Ozcelik and A. Nourhani and P.E. Lammert and V. H. Crespi and T. J. Huang},
	title = {Acoustic actuation of bioinspired microswimmers},
	journal = {Lab Chip},
	year = {2017}, 
	volume = {17},
	pages = {395--400}
	}
 	
@BOOK{K&K,
   author = "S. Kim and S.J. Karrila",
   title = "Microhydrodynamics",
   publisher = "Dover publication, Inc.",
   year = 2005,
   adress = "New York"
   }
   
@Article{Lippera2018,
	title = {No net motion for oscillating near-spheres at low ${R}e$ numbers},
	author = {K. Lippera and O. Dauchot and S. Michelin and and M. Benzaquen},
	journal = {J. Fluid. Mech},
	volume = {866},
	pages = {R1},
	year = {2019}
	}  
 
@Article{Mazur1974,
	author = {P. Mazur and D. Bedeaux},
	title = {A generalization of {F}ax\'en's theorem to nonsteady motion of a sphere through an incompressible 			fluid in arbitrary flow},
	journal = {Physica D},
	volume = {76},
	issue  = {2},
	pages = {235--246},
	year = {1974}
}

@Article{Nadal2014,
	author = {F. Nadal and E. Lauga},
	title = {Asymmetric steady streaming as a mechanism for acoustic propulsion of rigid bodies},
	journal = {Phys. Fluids},
	volume = {26},
	pages = {082001},
	year = {2014}
}

@article{Sabrina2018,
	author = {S. Sabrina and M. Tasinkevych and S. Ahmed and A.M. Brooks and M. Olvera$\;$de$\;$la$\;$Cruz 
	and T.E. Mallouk and K.J.M. Bishop},
	title = {Shape-Directed Microspinners Powered by Ultrasound},
	journal = {ACS Nano},
	volume = {12},
	number = {3},
	pages = {2939-2947},
	year = {2018}
	}

@article{Soto2016,
	author = {F. Soto and G. L. Wagner and V. Garcia-Gradilla and K.T. Gillespie and D.R. Lakshmipathy
	and E. Karshalev and C. Angell and Y. Chen and J. Wang}, 
	journal = {Nanoscale},
	year = {2016},
	volume =  {8},
	pages = {17788--17793},
	title = {Acoustically propelled nanoshells}
	}
	
@ARTICLE{Stokes1850,
   author = {Sir G.G. Stokes},
   title = {On the effects of the internal friction of fluids on the motion of pendulums},
   journal = {Trans. of the {C}ambridge {P}hil. {S}oc.},
   volume = {{I}{X}},
   year = {1850}
}
   
@article{Wang2014,
	author = {W. Wang and S. Li and L. Mair and S. Ahmed and T.J. Huang and
	T.E. Mallouk},
	title = {Acoustic Propulsion of Nanorod Motors Inside Living Cells},
	journal = {Nanomotors},
	volume = {53},
	pages = {3201--3204},
	year = {2014}
}

@ARTICLE{Burdick2008,
   author = "J. Burdick and R. Laocharoenshuk and P.M. Wheat and J.D. Posner and J. Wang",
   title = "Synthetic Nanomotors in Microchannel Networks: Directional Microchip Motion and Controlled
   Manipulation of Cargo",
   journal = "J. Am. Chem. Soc.",
   volume = 130,
   pages = "8164--8165",
   year = 2008,
   }

@ARTICLE{Campuzano2011b,
   author = "S. Campuzano and D. Kagan and J. Orozco and J. Wang",
   title = "Motion-Driven Sensing and Biosensing Using Electrochemically Propelled Nanomotors",
   journal = "Analyst",
   volume = 136,
   pages = "4621--4630",
   year = 2011,
   }

@ARTICLE{Doinikov1994b,
   author = "A.A. Doinikov",
   title = "Acoustic radiation pressure on a compressible sphere in a viscous fluid",
   journal = "J. Fluid Mech.",
   volume = 267,
   pages = "1--22",
   year = 1994
   }

@ARTICLE{Doinikov1996,
   author = "A.A. Doinikov",
   title = "Theory of acoustic radiation pressure for actual fluids",
   journal = "Phys. Rev. E",
   volume = 54,
   number = 6,
   pages = "6297--6303",
   year = 1996
   }

@ARTICLE{Ebbens2010,
   author = "S.J. Ebbens and J.R. Howse",
   title = "In pursuit of propulsion at the nanoscale",
   journal = "Soft Matter",
   volume = 6,
   pages = "726--738",
   year = 2010,
   }



@BOOK{Happel&Brenner,
   author = "J. Happel and H. Brenner",
   title = "Low Reynolds number hydrodynamics",
   publisher = "Martinus Nijhoff publishers",
   address = "The Hague",
   year = 1983,
   }

@ARTICLE{Hasegawa1969,
   author = "T. Hasegawa and K. Yosioka",
   title = "Acoustic radiation force on a solid elastic sphere",
   journal = "The Journal of The Acoustical Society of America",
   volume = "46",
   pages = "1139--1143",
   year = 1969
   }

@ARTICLE{Hasegawa1969,
   author = "T. Hasegawa and K. Yosioka",
   title = "Acoustic radiation force on a solid elastic sphere",
   journal = "The Journal of The Acoustical Society of America",
   volume = "46",
   pages = "1139--1143",
   year = 1969
   }

@ARTICLE{Ho1974,
   author = "B.P. Ho and L.G. Leal",
   title = "Inertial Migration of rigid spheres in two-dimensional unidirectional flows",
   journal = "J. Fluid Mech.",
   volume = "65(2)",
   pages = "365--400",
   year = 1974
   }

@ARTICLE{Riley1966,
   author = "N. Riley",
   title = "On a sphere oscillating in a viscous fluid",
   journal = "Quart. Journ. Mech. and Applied Math.",
   volume = "XIX",
   number = 4,
   pages = "461-472",
   year = 1966
   }

@ARTICLE{Rudnick1977,
   author = "I. Rudnick",
   title = "Measurements of the acoustic radiation pressure on a sphere in a standing wave field",
   journal = "The Journal of The Acoustical Society of America",
   volume = "62",
   number = 1,
   pages = "20-22",
   year = 1977
   }

@ARTICLE{Wang2012,
   author = "W. Wang and L.A. Castro and M. Hoyos and T.E. Mallouk",
   title = "Autonomous Motion of Metallic Microrods Propelled by Ultrasound",
   journal = "ACS Nano",
   volume = "6",
   number = 7,
   pages = "6122--6132",
   year = 2012
   }

@ARTICLE{Wang2013,
   author = "W. Wang and W. Duan. and S. Ahmed and T.E. Mallouk and A. Sen", 
   title = "Small power: Autonomous nano- and micromotors propelled by self-generated gradients",
   journal = "Nano Today",
   volume = "8",
   pages = "531--554",
   year = 2013
   }

